Measuring the Effectiveness of Privacy Policies for Voice Assistant Applications

Voice Assistants (VA) such as Amazon Alexa and Google Assistant are quickly and seamlessly integrating into people's daily lives. The increased reliance on VA services raises privacy concerns such as the leakage of private conversations and sensitive information. Privacy policies play an important role in addressing users' privacy concerns and informing them about the data collection, storage, and sharing practices. VA platforms (both Amazon Alexa and Google Assistant) allow third-party developers to build new voice-apps and publish them to the app store. Voice-app developers are required to provide privacy policies to disclose their apps' data practices. However, little is known whether these privacy policies are informative and trustworthy or not on emerging VA platforms. On the other hand, many users invoke voice-apps through voice and thus there exists a usability challenge for users to access these privacy policies. In this paper, we conduct the first large-scale data analytics to systematically measure the effectiveness of privacy policies provided by voice-app developers on two mainstream VA platforms. We seek to understand the quality and usability issues of privacy policies provided by developers in the current app stores. We analyzed 64,720 Amazon Alexa skills and 2,201 Google Assistant actions. Our work also includes a user study to understand users' perspectives on VA's privacy policies. Our findings reveal a worrisome reality of privacy policies in two mainstream voice-app stores, where there exists a substantial number of problematic privacy policies. Surprisingly, Google and Amazon even have official voice-apps violating their own requirements regarding the privacy policy.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> abstract.tex <==
\begin{abstract}
%Amazon Alexa 
%Voice is the most natural communication medium, Live-agent portals are introducing greater automation through speech recognition and text-to-speech technology turning on/off lights, playing music, we use the term skills to represent third-party voice apps including Amazon’s skills and Google’s actions , which serves as the first line of defense against malicious skills
Voice assistants (VA) are rapidly gaining popularity in performing everyday
tasks such as answering questions and placing online orders. 
With the emergence of the Amazon Alexa ecosystem, third-party developers are allowed to build new skills and publish them to the skills store, which greatly extends the VA's functionalities. 
Before a new skill becomes publicly available, that skill must pass a certification process which verifies that it meets necessary content and privacy policies. The trustworthiness of the skill publishing platform is of significant importance to platform providers, developers, and end users. 
Yet, we know little about whether the Amazon Alexa platform (which has a dominant market share) is trustworthy in terms of rejecting/suspending policy-violating skills in practice. %

In this work, we study the trustworthiness of the Amazon Alexa platform to answer three key questions: 1) Whether the skill certification process is trustworthy in terms of catching policy violations in third-party skills. 2) Whether there exist
policy-violating skills (\eg, collecting personal information from users) published in the Alexa skills store.
3) Once a policy-violating skill gets certified, how can possible adversarial developers increase the chance for their skill to reach end users?
We answer these questions by conducting a comprehensive measurement and data analytics study on the Amazon Alexa platform. 
Our key findings are threefold. First, we successfully got 132 policy-violating skills certified. Surprisingly, the certification process is not implemented in a proper and effective manner, as opposed to what is claimed that ``policy-violating skills will be rejected or suspended''.
Second, vulnerable skills exist in Amazon's skills store, and thus users (children, in particular) are at risk when using VA services. Third, skill discovery is potentially manipulable by adversarial developers in order to increase the success rate of skill hijacking. 
%In addition, we perform a preliminary measurement of the Google Assistant certification system, conduct a user study to understand users' misplaced trust  in VA platforms, and discuss how to enhance the trustworthiness of VA platforms.

%We also conduct a user study to understand VA users' concerns and expectations related to security and privacy.
%2) What are the users' complaints about existing skills available in the Alexa skills store and how do existing skills conform to the policy requirements? 4) What are the limitations of Alexa's policies and certification compared with \ja{the} Google Assistant platform?
\end{abstract}

%\begin{IEEEkeywords}
%	Voice assistants, Amazon Alexa, Trustworthiness
%\end{IEEEkeywords}

==> ccs-body.tex <==
\section{Introduction}

This is a sample!  It does not have a lot of fancy stuff in it, but if
you want to see a more complex sample, look at the original ACM
templates.

To fill up enough text to fill up 3 pages, we've included the CCS Call
for Papers three times.  It is always a good idea to include some
gratuitious citations to recent CCS papers~\cite{medvinsky1993netcash,
  bellare1993random, anderson1993cryptosystems, blaze1993cryptographic}.

\input{cfp}
\input{cfp}
\input{cfp}

\section{Conclusions}

In conclusion, it is rarely a good idea to include the same section three times in a paper, or to have a conclusion that does not conclude.

\appendix

\section{Location}

Note that in the new ACM style, the Appendices come before the References.

\input{cfp}

\begin{acks}
% TODO: For the submission, don't include acknowledgments since they would most likely deanonymize you.
\end{acks}


==> google.tex <==

\section{Comparative Measurement on Google Assistant Platform}\label{GoogleActions}

\iffalse 
\begin{table*}[h]
	\vspace{-6pt}
	%\captionsetup{font=scriptsize}
	\centering
	\resizebox{15.5cm}{!}{
		{%\Large
			\begin{tabular}{ | >{\centering\arraybackslash}m{1cm} | >{\centering\arraybackslash}m{12cm} | >{\centering\arraybackslash}m{2.3cm} | >{\centering\arraybackslash}m{2.3cm} | >{\centering\arraybackslash}m{1.1cm} |}
				\hline
				\rowcolor[gray]{0.5} \bf No. & \bf Policy & \bf Amazon Alexa & \bf Google Assistant & \bf Tested? \\
				\hline
				1 & Trademarks, Intellectual Property and Brands & $\medblackcircle$ & $\medcircle$ &  \\
				\hline
				2 & Spammy behavior: send excessive or irrelevant content. Drive traffic to a website
				or app.
				Submitting multiple duplicative Actions. & $\medblackcircle$ & $\medcircle$ &  \\
				\hline 
				3 & Web Search: The skill must search within a specific online resource, and
				cannot do a general web search, and must attribute the source of the information & $\medblackcircle$ & $\medcircle$ &  \\
				\hline
				\rowcolor[gray]{0.9} 4  &\multicolumn{4}{c|}{Child-directed skills}   \\
				\hline
				4.1 & It promotes any products, content, or services, or directs end users to engage with content outside of Alexa. & $\medblackcircle$ & $\medcircle$ &  \\
				\hline
			\end{tabular}
		}
	}
	\vspace{-6pt}
	\caption{\cltodo{summary of policy violations}}
	\label{table:simplepolicies}
	\vspace{-8pt}
\end{table*}
\fi 

%can put it in paper
%Key observation: There were exceptions in some cases where the skill that provides a response with a policy violation in the first session itself was accepted.
%Key observation: 
%\cltodo{ Completed: CW: please add or modify the motivation of this Google study. While our focus is on measuring the trustworthiness of Amazon Alexa platform, we also briefly evaluate how rigorous is the certification system in Google Assistant. }
%With this preliminary study on Google, our purpose is not to draw a conclusion that Alexa's certification is comparatively lax or strict.
While our primary focus is on the study of Amazon Alexa platform, we conducted a preliminary measurement on Google Assistant platform as well. We submitted \clnote{273} policy-violating actions (listed in Table~\ref{table:policies} of Appendix~\ref{AppendixA} and Table~\ref{table:requirement} of Appendix~\ref{AppendixAA}) to observe if they can pass the certification. 
%This preliminary comparative study helps us to understand how Amazon's certification differs from Google's.}

%for the skills we published on the Alexa's skills store
In terms of development, both Google actions and Alexa skills are similar to each other in their structures. Out of the few differences, a notable difference between the two is that Amazon requires developers to provide a developer privacy policy only when the skill explicitly states that it collects personal data. For other skills, it is not mandatory to provide one. 
%Google requires an action-specific privacy policy for every action whereas
%The developer privacy policy in Alexa is normally a general privacy policy of the developer or an organization for all its services. It doesn't provide a clear statement of what the particular skill is capable of doing. 
On the contrary, Google mandates that a privacy policy specific to each action must be provided. This gives the end user a better understanding rather than a generic long document that may or may not reflect what the action does.
We used \clnote{14} Google cloud platform accounts for our experiments due to the projects quota limit imposed by Google.

\subsection{Google Assistant's Certification}
%\cltodo{how did you choose the ten actions you submitted from the 112+ skills?} Google calls these skills as kids \& family skills.
\subsubsection{Actions for Families/Kids}
Actions for families is Google's program for family-friendly actions that engage the whole family. We submitted 85 actions that violate policy guidelines specific to actions intended for children. While 70 of these actions were rejected, 15 actions did pass the certification. We specifically focused our experiments on actions that {\em collect personal information from children} since it is restricted by COPPA regulations and actions that {\em contain content not suitable for kids or had advertisements} (\ie, policies 2 and 11.b in Table~\ref{table:policies}). While most of these actions were rejected, we were still able to certify actions that violate COPPA regulations and had advertisements. From our experiment results, we could infer that Google has a strict certification procedure for actions for families but it is still not completely capable of rejecting all malicious actions.  %\cltodo{Check and rewrite: These were the exact same copies (in content) of the skills that were published on Alexa's skills store. \clnote{XXX} of these actions were capable of responding with a policy-violating response while 1 action was a benign action with no policy violation. Google rejected all \clnote{XXX} policy-violating actions while the benign one was certified. We changed the back-end code of this action (\ie, Fun kid facts) after certification to test the content changing attack on Google actions. We included a malicious policy-violating response and this change was immediately deployed to the live action without needing a re-certification thus resulting in a live action targeted to families available in the assistant directory having the same policy-violating response that was in the other actions that were rejected. We immediately removed the policy violation right after the short testing to make sure no actual users had been affected.}
%\cltodo{Check and rewrite: Out of the 10 actions, Bedtime Tales was a storyteller action while the other 9 were fact providing actions. Bedtime Tales collected the user's name and read out a personalized story as the response. It was rejected citing the reason as ``breaking the actions for families policies that prohibits collecting personal information from children''. We re-submitted the action by explicitly asking just the first name which is allowed as per the COPPA (details in Sec.~\ref{sec:COPPA}) regulation but even this led to a rejection. In both cases, the actions were capable of collecting only the first name from the user and not the full name. Out of the 9 fact actions that were submitted, only the one that had no malicious response got certified. All the 8 rejections cited the reason that the action did not contain children level educational material. }

%and also follows the COPPA regulations

\subsubsection{Bypassing Certification}
We submitted 273 policy-violating actions in total out of which 116 actions were certified and 157 never passed certification. Out of this, 101 actions were certified into the general category. Some actions required a re-submission to be certified. To bypass the certification system, we added the malicious response to a large number of possible responses so that the certification team would not encounter it by limited voice checking. The second method we used to bypass the certification stage was to ask for personal information indirectly. Rather than asking a user his/her name or age directly we could use a simple math trick that allows us to infer the age or casually add a "What should we call you?" at the later stages of an action's functionality. 87 actions that we submitted to the general category could never pass certification even after we used these bypassing techniques. 
We got multiple rejections stating reasons such as an invalid privacy policy or violation of intellectual property related policy. After making the necessary changes, all of these actions were certified and published to the assistant directory (\ie, general category) on re-submission. In order to test its applicability in Amazon, we made the same inconsistency/mismatch in Alexa skills and submitted it. Some examples are giving the wrong skill name in the privacy policy and using the word action instead of skill in the description. But Amazon certification team did not find a problem with these errors and certified all the skills. 
%We never received some of the feedback reasons that we got here from Amazon. 
%We did not try to submit the Bedtime tale action to any other category because the policy (\ie, collecting personal information) that it violates is only applicable to actions for families category.
%Table~\ref{table:comparison} summarizes the comparative study results.
Google also could identify spam actions and reject them if an action is a duplicate of another action in the directory while Amazon does not detect this. 
While Google does do a better job in the certification process based on our preliminary measurement, it is still not perfect and it does have potentially exploitable flaws that could lead to malicious actions being available in the Assistant directory. Since our primary aim was just to compare the certification system, we did not look for more advanced methods to bypass this system. 
%\cltodo{Christin: we may extend the conclusion??}

\begin{figure} [h!]
	\begin{center}
	\vspace{-5pt}
		\includegraphics[width=0.48\textwidth]{./figures/actionfeedback.png}
	\end{center} \vspace{-10pt}
	\caption{Certification feedback from Google Assistant showing the inconsistency in certification.}\vspace{-10pt}
	\label{actioncertificationfeedback}
\end{figure}

\subsubsection{Inconsistency in Certification Feedback}
From our experiments we noticed that there were a lot of inconsistencies (same as in Amazon Alexa) in the feedback provided by the certification team after the submission of actions. In some cases, the action failed in certification while in others the same action passed certification even though there was no change in the content of the actions and contained a malicious response both times. In some other cases, the actions were rejected citing different reasons. An example of inconsistency in feedback is shown in Fig.~\ref{actioncertificationfeedback}.




\subsubsection{Dynamic Testing}
Only 76 actions were available in the families/kids category of Google Assistant platform as of April 2020. 
We performed a dynamic testing on all these actions. This number is very less compared to that of the skills available in Alexa's skills store. The low number of actions for families can be a result of the stricter certification system. Note that the actions we submitted are not included in this number. We found one problematic action called "Smallfoot" that asks the user's name. In addition, the URL provided as the action's privacy policy does not lead to a webpage that contains a privacy policy but rather to a page advertising the company's products. Thus the user's personal data is being collected without informing them of the action's data practices. 

\subsubsection{Post-Certification Vulnerability}
Similar to Alexa skills, content changing attack can be performed on Google actions as well. The back-end of an action can be updated after the certification and this will not require a re-certification to be made available in the production version. The Google Assistant platform has entities that denote the type of data that can be collected by a placeholder (which works similar to slots and slot types in the Alexa platform). The entity \texttt{sys.any} can be used to store all kinds of data. By changing the content of the question in the back-end after certification, an action that uses this entity can collect any kind of information including personal information from the response provided by users. Thus the developers do not have to create a custom entity to collect the personal information they require.


%Possibly outsourced and not conducted in the US.

\subsection{Feedback Time for Certification}
It is interesting that Amazon Alexa and Google Assistant platforms exhibited different patterns in terms of the certification feedback time.   
Fig.~\ref{fig:feedbacktime}(a) shows the CDF (cumulative distribution function) of time taken to receive a feedback for skill/action certifications. For skill submissions, in most cases, we received the certification feedback within 24 hours. The certification process of Google actions took varying amounts of time. For our first 10 submissions in 2019, most certification results were received within 1-2 days (one case took 3 days and another case took 7 days to get the feedback). However, for our recent submissions from February to April 2020, the certification feedback was received much faster. About 10\% of the actions took less than 10 minutes to get a feedback. 

Fig.~\ref{fig:feedbacktime}(b) plots randomly selected 200 timestamps when we received certification feedback emails from Amazon Alexa and Google Assistant platforms, respectively. These timestamps are sorted by EST time. In most cases, feedback emails we received from Amazon had timestamps between {11:40pm} and {8:37am} EST. Since there are no certifications happening at any time other than this specific time range, it is likely the feedback emails were sent either by an automated process (but evidence shows that the skill certification was largely performed in a manual fashion) or sent manually by an outsourced certification team. Actually, we were contacted by an Amazon employee based out of the US to help us in publishing a skill that was rejected multiple times on submission.
In this case, it is very important that the team is made aware and given proper training about the policies in place, to ensure that the skill doesn't break any policies specified by Alexa platform. From our experiments, we were able to understand that the certification team may not be properly aware about the COPPA~\cite{Apthorpe:2019:COPPA} regulations because many of our certified skills did not comply with COPPA. These skills were not hiding a policy violation or delaying it and had a violation in the \texttt{LaunchIntent} itself thus confirming the lack of awareness. 

For Google actions, the feedback mails for all the actions we submitted this year were received between 10:51am and 1:19am EST (in most cases, it was between 8:00am and 7:00pm PST, as shown in Fig.~\ref{fig:feedbacktime}(b)). This indicates that the Google certification team possibly works based on the US timezone, as opposed to the Alexa's certification team.
%in the various countries that the skill is intended for

\begin{figure}[!htb]
	\vspace{-10pt}
	\centering
	\subfigure[Time taken to receive feedback]{\includegraphics[width=0.49\columnwidth, height=2.9cm]{./figures/cdf.pdf}\label{eva:pattern:spm}}
	\subfigure[Time when getting feedback]{\includegraphics[width=0.49\columnwidth, height=2.9cm]{./figures/dots.pdf}\label{eva:pattern:sc}}\vspace{-12pt}
	\caption{Feedback time for certification.}
	\label{fig:feedbacktime}
		\vspace{-15pt}
\end{figure}

%These results show that Google did take extra measure for the actions for families program in order to provide a better experience for families. 



%\begin{figure} 
%	\begin{center}%\vspace{-15pt}
%		\includegraphics[width=5cm]{action.jpg}
%	\end{center} \vspace{-16pt}
%	\caption{A live action giving guidance on how to create or build a dangerous material (silencer).}
%\end{figure}

\subsection{Comparative Analysis of Policies}\label{sec:ComparativeAnalysisPolicies} 
%\cltodo{shrink to two paragraphs contrasting policies}
%There has been no rigorous way to assess the completeness and quality of security policies~\cite{Security:2019:COPPA}. 

The completeness and quality of policy requirements are also important to achieve a trustworthy VA platform. While both Amazon Alexa and Google Assistant claim that they reserve the rights to reject voice apps on the basis of content or functionality that are not explicitly prohibited by their policies, a lack of explicit restrictions on certain behaviors leaves room for dispute by developers. We conduct a comparative analysis to understand how Amazon's policies differ from Google's and its possible limitations. 
%Our analysis reveals potential weaknesses of policy requirements in Alexa. 

%\cltodo{Appendix, show details} 

%One notable area where Amazon does not explicitly restrict content is in regards to duplicate skills. To address this challenge,

{\bf Policy coverage.} 
Amazon Alexa has specified 7 privacy requirements~\cite{PrivacyRequirements} and content policy guidelines~\cite{PolicyTesting} which
are categorized into 14 main sections (where the detailed list is in Appendix~\ref{AppendixA}). These privacy requirements and policy guidelines have certain overlaps, \eg, both highlight that collecting personally identifiable information is not allowed. By comparing with policies for Google Assistant~\cite{PolicyGoogleActions} (which have 19 sections for content restrictions), we find that Amazon specifies fewer policies in multiple aspects. 
Here we discuss two notable sections of policies that are missing in Alexa. 

%For instance, a developer would be able to claim that an "unreasonably long" audio clip is in fact reasonable in the context of their skill's use, and the lack of an explicit criterion for "unreasonably long" – 240 seconds in Google's case – makes it difficult for Amazon to dispute the developer's assertion. 
% such as sensitive events.While Amazon may indeed attempt to filter out such skills during the vetting process, 

%\cltodo{better give a number how many more policies in Google, and their overlap}. We give an 
{\em Sensitive events.} Google Assistant prohibits the publication of actions that ``lack reasonable sensitivity towards, or capitalized on, a natural disaster, atrocity, conflict, death, or other tragic event,'' while Amazon Alexa makes no such restriction. Such a policy should be explicit, as references to tragic events may be traumatic for users who were affected by such events. In fact, a user reviewed the ``Amazon Story time'' on the skills store with ``want your kid to hear a Boston Bombing story?''. It is crucial to bear in mind all potential Alexa users, and as such a policy disallowing offensive views on tragic events should be added into Alexa's existing policies. 

%By prohibiting such intents from being created, the vetting process may eliminate this possibility entirely without the need to carefully read every line of Action code. whereas a harmful intent may not be detected during Amazon's certification process. Any irrelevant intent, harmful or not, is expected to be rejected.} Such irrelevant intents are an area where a harmful developer could hide malicious code. 
%Amazon Alexa does not explicitly prohibit the creation of intents within a skill that are misleading or irrelevant to the overall skill. This section in

{\em User experience.} Google Assistant includes policies such as: i) an Action claims supporting a larger scope of commands than it actually does, ii) audio not matching visual text, and other aspects which may harm user experience. {Amazon does not specify these user experience policies in the certification requirements} and this may consequently weaken the overall experience of users.

%listening for a user command without a prompt, listening to users without implicit or explicit prompts or misguiding users about the nature of an interaction, playing silent sound files without a clear purpose, continuously playing text-to-speech or recorded audio for unreasonable amounts of time, 
%The Google Action Store's policies also has a section on user experience which the Alexa skill Store appears to lack. 


%Amazon does not have a policy requiring developers to gain explicit consent from the user before collecting Email Addresses. Requiring consent from users before collecting emails is a standard practice in many app stores including Google's Action Store, and helps protect users' security by preventing the collection of personal data without consent. Amazon lacks this requirement and consequently weakens the security of all its users' private data.

%Amazon also lacks policies dealing with one skill interacting with other skills without the user's consent. Google prohibits their Actions from having security vulnerabilities that can be exploited to compromise another Action, and also prohibits Actions from running other Actions without user consent. Amazon lacks such policies, implying that skills are allowed to access other skills without the user's knowledge. If a malicious skill was capable of accessing a private skill such as a bank skill (e.g. Capital One), a developer might be able to access the user's bank information, which would be a serious breach in privacy and security.

%\cltodo{rephrase: avoid misleading conclusion, This does not imply that Amazon Alexa’s policy gives more freedom, but I agree that it can be more ambiguous.}

{\bf Policy details.} Amazon Alexa's policies also lack as much detail when compared to those of Google. For instance, both platforms prohibit ``promoting violence and dangerous activities, such as organized crime, terrorism, and unsettling content or extreme gore''. Google's policies continue to explicitly restrict the promotion of self-harm, as well as the promotion of bullying and harassment. While one might argue that these are implicit in Amazon, Alexa's policies regarding ``violence'' are nonetheless ambiguous with regards to self-harm and bullying, and as such can be strengthened by adding clear statements disallowing such behaviors.

{\bf Duplicate content is allowed.} Google prohibits ``submitting multiple duplicative Actions to the actions directory'', while Amazon lacks any mention of duplicate skills (including front-end interfaces and back-end code). In our experiments, we were successful in submitting multiple identical skills, and both skills were live simultaneously. As a consequence, Alexa's skills store is at risk of being bloated by a number of duplicate skills. 
%If a malicious skill is accepted initially through the vetting process, it may be possible for a developer to submit multiple versions of the same malicious skill, such that even if one skill is retroactively removed for being malicious, other exact copies may still exist undetected on the store. 
%In addition, the duplicate naming (\ie, multiple skills having the same name) in Alexa is problematic. Despite providing more options to developers, it may hurt the reputation of legitimate developers if poorly designed skills use identical names as well-designed popular skills. Amazon's lack of restriction on duplicate invocation names gives malicious developers an avenue to attempt to "hijack" a skill name and have users unknowingly install harmful skills with the same names as legitimate skills.
%It may be possible for a malicious skill to become prioritized by voice-based installation without the user's knowledge (\ie, voice-squatting attacks~\cite{Security:2018:Squatting, DangerousSkills:2019}). 

% While two identical skills can be submitted to Alexa's skills store, it is also possible for two drastically different skills with identical invocation names to be submitted. While one developer could have a legitimate, non-problematic skill, another malicious developer may have a skill with an identical name that causes trouble or harm to a user's privacy or security.
%\noindent{\bf Duplicate invocation names.} Alexa's skills store has no restrictions on multiple skills having the same name.

%A lack of restriction on the duplicate skills in itself may not be malicious, but it is still significantly problematic because it makes it more difficult to discern malicious skills among a large number of similar or identical-looking skills.

%(2) Duplicate naming in Alexa is an involved challenge. Despite providing more options to developers, it may hurt the reputation of legitimate developers if poorly designed skills use the same names as well-designed popular skills. 

%\begin{tcolorbox}[colback=lightgray!5,colframe=lightgray!40!gray,title={Duplicate skills}]
%	By extension of the previous weakness
%\end{tcolorbox} Security Implication:


%\cltodo{both Amazon and Google have no requirement on full profile of a developer, which violates COPPA, which provides}

%\section{Amazon Alexa vs Google Assistant}

==> review.tex <==

\section{Paper Reviews From IEEE S\&P 2020}\label{AppendixReview}
We attached the reviews that we received from S\&P’20, along
with information about the way we have addressed them in this
paper. We got all three "weak accepts" in late Feb 2020, which was the end of S\&P20’s review cycle. 
Unfortunately, this paper was not accepted by S\&P’20.
These reviews were helpful for us to improve our paper. 
Note that we attached a concise version (with main limitations) of reviews from S\&P’20.

\subsection{Reviewer A (Weak accept)}
{\bf Strengths:} i) The paper is interesting, original, and timely since there are current many concerns about voice assistants. ii) The paper is rich in experiments and analyses that help the reader to understand the trustworthiness from different perspectives: they managed to get hundreds of so-called dangerous skills certified, they found existing dangerous skills, and they measured user perception of trustworthiness through a user study.

\vspace{3pt}
\noindent{\bf Limitations:}\\
\noindent {\bf (A1)} \clnote{I recommend emphasizing the fact that skills backend code is a black box for the certification process. }\\
{\bf Response A1}: We have emphasized it in Sec.~2.

{\bf Jeffrey A1}: We address this concern in Sec.~2 by adding more emphasis to the fact that the backend code is hidden from the certification team during the certification process. 

\vspace{3pt}
\noindent {\bf (A2)} \clnote{The paper contains a preliminary analysis of the Google Assistant platform; however, the number of skills tested is too small to make any proper generalizations.  Having a comparable set of experiments may help support these generalizations and better understand if/why the Google Assistant certification is better.}\\

{\bf Response A2}: In our previous version, we only submitted 10 policy-violating Google actions. In this paper, we have significantly extended the measurement of Google Assistant platform to better understand its certification system. We submitted 273 policy-violating actions in total out of which 116 actions were certified and 157 failed to pass the certification. Our measurement on Google Assistant platform shows that it also has potentially exploitable flaws. In addition, we also submitted more policy-violating skills and successfully got these skills certified.

{\bf Jeffrey A2}: In the previous version of this paper, we submitted 10 policy-violating Google actions. In our revised version, we have significantly extended the measurement of Google Assistant platform actions to better understand the certification process. Furthermore, we submitted 273 policy-violating actions in total out of which 116 were certified and 157 failed to pass the certification. Our measurement on the Google Assistant platform shows that it also has potentially exploitable flaws. 

\vspace{3pt}
\noindent {\bf (A3)} \clnote{It is also not clear why the lack of policy details is necessarily a bad thing.  The paper states that both Amazon Alexa's and Google assistant policies prohibit "promoting violence", then Google details specific examples of "promoting violence", while Amazon Alexa's does not. This does not imply that Amazon Alexa's policy gives more freedom, but I agree that it can be more ambiguous.}\\
{\bf Response A3}: We agree. We have rephrased the sentences to avoid any misleading conclusion in Sec.~\ref{sec:ComparativeAnalysisPolicies}.  

{\bf Jeffrey A3}: We agree with the reviewer and have rephrased the misleading sentences in Sec.~\ref{sec:ComparativeAnalysisPolicies}. 

\vspace{3pt}
\noindent {\bf (A4)} \clnote{The end of section V.D discusses some strategies to improve the trustworthiness of the skill certification process. However, the discussion lacks pros and cons of each strategy, especially their feasibility/cost in the current context and what system assumptions have to be changed to make them possible. I suggest addressing these concerns.}\\

{\bf Response A4}: We have added the discussion about the pros and cons of each strategy in Sec.~\ref{Mitigation}.    

\subsection{Reviewer B (Weak accept)}
{\bf Strengths:} i) Practical demonstration of an important problem in widely-used systems. ii) Not just a narrow exploit, demonstrated with a large number of cases.
iii) Includes good discussion of ethics, implications, etc.

\vspace{3pt}
\noindent{\bf Limitations:}
\noindent {\bf (B1)} \clnote{I think this is an interesting and informative paper that is very practical and relevant. My main complaint is that the authors may be trying to do too much in one paper. Perhaps this could be addressed with a table or figure up front that presents and overview of what is going to be presented.}\\

{\bf Response B1}: Our main focus is to measure whether the skill certification process is trustworthy in terms of catching policy violations in third-party skills. We have removed the user review analysis part. We list the key research questions in Sec.~\ref{Introduction}.

{\bf Jeffrey B1}: Our main focus is to measure whether the skill certification process is trustworthy in terms of catching policy violations in third-party skills. We have removed the user review analysis section and listed the key research questions in Sec.~\ref{Introduction}.



\subsection{Reviewer C (Weak accept)}
{\bf Strengths:} i) The paper is the first to explore the extent to which privacy-violating skills that are intentionally authored as such were violated. ii) This paper covers an important topic in a relatively under-explored area. It also has some important findings, specifically that Alexa skills often violate user privacy.

\vspace{3pt}
\noindent{\bf Limitations:}\\
\noindent {\bf (C1)} \clnote{The paper meanders, however, into tangents such as legal analysis (e.g., on COPPA) where the authors are unqualified to offer legal opinions.}\\

{\bf Response C1}: We have rephrased the sentences to avoid offering any legal opinions in Sec.~\ref{sec:COPPA}.  

{\bf Jeffrey C1}: We have rephrased any sentences in Sec.~\ref{sec:COPPA}, which may have offered legal opinions or analysis.  

\vspace{3pt}
\noindent {\bf (C2)} \clnote{The section on mitigation in similarly non-technical and uninformative. The suggestions are trite (e.g. "ensure description to function fidelity", which essentially says nothing more than making code match spec... OK, but that's a hard problem that software engineers have been studying for decades).}\\
{\bf Response C2}: The mitigation is not our focus in this paper. We just discuss several research solutions that can improve the security of third-party skills.   

{\bf Jeffrey C2}: Mitigation is not the focus of this paper. However, we do discuss several research solutions that can improve the security of third-party skills, yet we leave the implementation of these solutions to future research efforts.   

\vspace{3pt}
\noindent {\bf (C3)} \clnote{This is a good problem area. The authors should be more rigorous in both the text analysis of the reviews, as well as in the dynamic testing; for an example of dynamic testing in this area, the authors might look at recent work from Northeastern, or the IoT Inspector project, both of which have done similar testing of IoT devices (including Alexa), as far as third-party data leaks.}\\
{\bf Response C3}: The "text analysis" is about the user review analysis in our previous version. We have removed this part. For our dynamic testing of skills, it is quite different from existing works in traditional software testing. We have checked out these two projects mentioned by Reviewer C. The IoT Inspector is an open-source tool to analyze the IoT network traffic. The dynamic testing work from Northeastern focuses on identifying software bugs in IoT firmware. While the objective of our preliminary dynamic testing of skills is to find any policy violating skills (possibly as consequences of a lenient certification system) in a conversation between users and the Alexa device, which is different from these two projects.

{\bf Jeffrey C3}: The "text analysis" is about the user review analysis in our previous version. We have removed this section. For our dynamic testing of skills, it is quite different from existing works in traditional software testing. We have examined the two projects mentioned by Reviewer C. The IoT Inspector is an open-source tool to analyze the IoT network traffic. The dynamic testing work from Northeastern focuses on identifying software bugs in IoT firmware. While the objective of our preliminary dynamic testing is to find policy violating skills (possibly as consequences of a lenient certification system), this differs greatly from the dynamic testing outlined in both suggested examples.


==> skilldiscovery.tex <==


\section{Understanding the Skill Discovery Process}\label{sec:discovery}
%\section{Demystifying Skill Discovery Process}  

%\cltodo{* I'm not totally sure what you mean by "post positive reviews and ratings."  Can you provide more detail on exactly what you did?  Is it possible that you caused a user to be exposed to a skill (even a benign one) that they would have preferred not to be exposed to?  Is it possible that you impacted those offering skills, particularly if Alexa effectively recommends skills in a winner-takes-all manner?    Did you pass this aspect of your study by your IRB?}

%We next investigate how possible an adversary may leverage the lenient skill certification process to reach end users in the Alexa ecosystem. \eg, remove a {stain type} stain

%Auto-enablement means that you can use a skill immediately when you say, “Alexa, open [the skill].”

%We have demonstrated that malicious third-party skills can easily bypass the certification process and become available in the skills store. 

In this section, we seek to understand the third-party skill discovery process. By default, VA providers find a native skill to fulfill the spoken requests from users. When there are no native skills available, the request will be sent to a third-party skill~\cite{arXiv:review:2019}. Voice-squatting attacks based on speech misinterpretation~\cite{DangerousSkills:2019, Security:2018:Squatting} only provide the possibility that a malicious skill impersonates a legitimate one. The success of such squatting attacks depends on the skill discovery/recommendation algorithm of VA platforms. However, it is undisclosed how Alexa chooses one of the skills with similarly pronounced invocation names. Alexa's name-free interaction~\cite{SkillDiscovery} makes skill discovery more complicated.
Instead of calling the skill by its invocation name, users can just tell Alexa what they need. Then, the machine-learning based skill discovery module will first find the most statistically significant (k-best) matches of candidate skills, and then select the most relevant skill by taking multiple factors into account including a skill's quality and usage. We examine how different factors (\eg, user review and rating) may affect the outcome of skill discovery if there are conflicts/ambiguities with names for skill invocation. If external factors and parameters can influence the skill discovery process, adversarial developers may manipulate these factors (\eg, by posting fake reviews) to increase the chance that a malicious skill reaches end users. 
 



%which can be potentially exploited by malicious developers to an adversarial skill reach end users after a malicious skill has been certified on Amazon Alexa platform.


 %considering contextual signals (\eg, customer satisfaction including number of customers, customer engagement, and ratings).
 
 %which skill can provide the most likely correct response from an invocation name-free utterance.
 
%Some of the criteria we use to choose auto-enabled skills include customer satisfaction, such as number of customers, customer engagement, and ratings, as mentioned above.


%For example, for a malicious skill where its invocation name carries similar phonetic pronunciation with a well-designed one, we test whether the malicious skill is able to hijack the well-designed one by manipulating these factors. In addition, we seek to uncover new vulnerabilities in VA platforms through a comprehensive security assessment. 

\subsection{Methodology}

%We designed an experiment to understand Alexa's third-party skill discovery process. 
%Fig.~\ref{skilldiscovery} shows the experiment setup for demystifying the skill discovery process on the Amazon Alexa platform.
%varied the number of user reviews and ratings for these skills, and


We first identified existing skills carrying the same or similar phonetic pronunciation invocation names. We then observed whether a particular skill is constantly discovered by Alexa. For this experiment, we focused on matching by the invocation name where the user explicitly asks to open a certain skill. The enabling by voice feature was used for this process. The Alexa smartphone app was used to monitor the skill enablements.


%\begin{figure} [h]
%	\begin{center}\vspace{-6pt}
%		\includegraphics[width=0.45\textwidth]{./figures/skilldiscovery.pdf}
%	\end{center} \vspace{-5pt}
%	\caption{Experiment setup for demystifying the skill discovery process in Amazon Alexa platform.}\label{skilldiscovery}
%	\vspace{-12pt}
%\end{figure} 

%\cltodo{Christin: what are the skill names, show Case Study???}\\ Alexa responds by enabling a skill with the invocation name without providing any information or asking for confirmation from the user regarding whether it is the right skill being enabled other than reading out the skill’s public name.


For this experiment, we collected skills that have identical invocation names from the skills store.
We logged into a new Amazon account and opened each of these skills by saying “Alexa, open <invocation name>”. We did not enable any of these skills beforehand. After a skill is enabled,  the same skill is opened for every invocation until it is explicitly disabled. Interestingly, from the results we encountered, the skill that was enabled was the one with the highest number of reviews/ratings in the store.
Then we disabled that skill. On the next attempt at opening a skill with the invocation name, a new skill with the same invocation name was enabled. This was the skill that was second in terms of ranking based on the number of ratings/reviews. For invocation names that have more than 2 skills published on the store, we did the above process a third time. 
After making a note about the skills and the orders in which they were enabled, we logged into two other Amazon accounts and repeated the same experiment. We found that the skills that were enabled and their ordering was the exact same on every account. 


\begin{table}[hbt!]
	\vspace{-10pt}
	%\captionsetup{font=scriptsize}
	\centering
	\resizebox{8.2cm}{!}{
		{%\Large
			\begin{tabular}{ | >{\centering\arraybackslash}m{2.3cm} | >{\centering\arraybackslash}m{2.5cm} | >{\centering\arraybackslash}m{1.0cm} | >{\centering\arraybackslash}m{2.0cm} | >{\centering\arraybackslash}m{1.0cm} |}
				\Xhline{3\arrayrulewidth}
				%\toprule[2.0pt]
				 \rowcolor[gray]{0.9} \bf Skill Name & \bf Developer & \bf Rating & \bf Total Reviews & \bf Order\\
				
				\hline
				 \multirow{2}{*}{Zipcode lookup} & dogmarcopolo & 3.6 & 904 & 1  \\
				 \cline{2-5}
				 & GPDL Industries & 4.3 & 10 & 2 \\
				\hline
				
				 \multirow{2}{*}{Yoga music} & Zen apps & 4.1 & 14 & 1  \\
				\cline{2-5}
				 & App316.com & 4.4 & 6 & 2 \\
				\hline
				
				 \multirow{2}{*}{Yo mama jokes} & Franks \& Beans & 4.2 & 2020 & 1  \\
				\cline{2-5}
				  & Per4mnce Software & 4.2 & 168 & 2 \\
				\hline
				
				\multirow{2}{*}{Yes man} & Dawson Foushee & 3.6 & 16 & 1  \\
				\cline{2-5}
				 & Naitian Zhou & 3 & 1 & 2 \\
				\hline
				
				\multirow{2}{*}{\shortstack[c]{World war \\ two trivia}} & Mustang D & 4.4 & 113 & 1  \\
				\cline{2-5}
				  & Jobo’s Rum & 1.9 & 2 & 2 \\
				\hline
				
				\multirow{2}{*}{World history} & Appbly.com & 3.4 & 51 & 1  \\
				\cline{2-5}
				  & Mudit Surana & 1.5 & 3 & 2 \\
				\hline
				
				\multirow{2}{*}{Work time tracker} &Alex & 3.2 & 10 & 1  \\
				\cline{2-5}
				 & estherleah & 0 & 0 & 2 \\
				\hline
				
				\multirow{2}{*}{Wine expert} &Lavigilanta.info & 1.3 & 7 & 1  \\
				\cline{2-5}
				 & Aletheia & 0 & 0 & 2 \\
				\hline
				\multirow{3}{*}{Who goes first} & Christopher Pierce & 3.2 & 56 & 1  \\
				\cline{2-5}
				 & Novavux & 3.3 & 4 & 2 \\
				\cline{2-5}
				 & ProfDeCube & 0 & 0 & 3 \\
				 
				\hline	
				\multirow{3}{*}{Weird facts} & Venkateswara Rao & 3.9 & 169 & 1  \\
				\cline{2-5}
				 & Baujaco &3.3 & 10 & 2 \\
				\cline{2-5}
				 & Supermann & 4.5 & 5 & 3 \\
				\hline	
		
				\Xhline{3\arrayrulewidth}
			\end{tabular} 
		}
	}
\vspace{0pt}
	\caption{List of skills in our measurements.}\label{table:discoveryprocess1}
\vspace{-18pt}
\end{table}


\subsection{Experiment Results}
Table~\ref{table:discoveryprocess1} shows the list of skills in our measurements to understand the skill discovery process. Our measurements reveal that: i) the priority first goes to the skill that is already enabled on the device; and ii) skill discovery is likely a function of user reviews and ratings. The second priority goes with the skill that has the highest number of reviews and ratings. The user’s opinion about which skill to enable is neither asked for nor is the user properly informed about the particular skill other than to just state the ``public name'' of the skill when it is enabled. To enable a skill that comes later in the ranking, it has to be enabled either by visiting the skills store or by multiple enabling and disabling of skills.

After a malicious skill is certified and published in the skills store, an attacker may post fake positive reviews and ratings to increase the success rate of skill hijacking. Since there are very few skills that have a sizable number of reviews, in many cases the number of required fake reviews that an attacker needs to post can be considerably less. Also, the users would not know which skill they are using unless they check their Alexa companion apps on their mobile devices.
We recognize that Amazon's fraud detection mechanisms may catch fake reviews. However, the longstanding problem of preventing the manipulation/inflation of usage statistics makes it probable for the adversarial developers to manipulate the skill discovery~\cite{Yao:2017:ACA}. For example, Amazon stated that there exists fake reviews designed to evade detection, and review abuse continues, despite the company's efforts~\cite{AmazonFakeReview}. 
The poor certification process combined with potentially manipulable skill discovery puts daily VA users at high risk. 



%* I disagree with your assertion "We ... revealed that an adversary may manipulate the skill discovery mechanism to hijack benign skills."  Your results suggest that an adversary could hijack this mechanism *if the adversary can inflate the number of ratings and reviews.*  Unless I misunderstood something, I don't believe you demonstrated that Amazon's fraud detection mechanisms are insufficient to catch this.  I think it would be fine just to say that you provided details about the skill discovery process Amazon uses to recommend skills, which is a nice finding on its own. [CL: rewrite]


%This motivates us to perform a user-centered study in Sec.~\ref{sec:User} to understand VA users' concerns and identify potential privacy issues in existing skills. 



%Our research plan is to identify factors that may influence the skill discovery process, and explore other possible means to boost voice-squatting attacks.
%Our measurements reveal that: i) the priority first goes to the skill that is already enabled on the device; and ii) the skill discovery is a function of reviews and ratings. The second priority goes with the skill that has the highest number of reviews and ratings. Unfortunately, combating against manipulating or inflating usage statistics is a long-standing unsolved problem [???]. This indicates that the skill discovery is manipulable by adversarial developers. After a malicious skill is published, we found that injecting fake positive reviews and ratings can greatly increase the success rate of skill hijacking.











\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%
<    Amazon introduced Canfulfillintentrequest which are keyword and phrase tags that developers can add to make their skills easier for Alexa to find when responding to generic requests by users. This method is used when the user doesn’t explicitly ask for a particular skill but asks for a particular functionality. Amazon terms this "nameless invocations”.   needed?     >

For this experiment, we focused on matching by the invocation name where the user explicitly asks to open a certain skill. The enabling by voice feature was made use of for this process. The Alexa app was used to monitor the skill enablements.

Initially, we collected skills that have identical invocation names from the dataset.
We logged into a new Amazon account and opened each of these skills by saying “Alexa, open <invocation name>”. We didn’t enable any of these skills beforehand.
Alexa responds by enabling a skill with the invocation name without providing any information or asking for confirmation from the user regarding whether its the right skill being enabled other than reading out the skill’s public name. After this step, until the skill is explicitly disabled, the same skill is opened for every invocation. Interestingly, from the results we encountered, the skill that was enabled was the one with highest number of reviews/ratings in the store.
Then we disabled the skill. On the next attempt at opening a skill with the invocation name, a new skill with the same invocation name was enabled. This was the second skill in terms of ranking based on the number of ratings/reviews. For invocation names that have more than 2 skills published on the store, we did the above process a third time. 
After noting down the skills and the orders in which they were enabled, we logged into two other Amazon accounts and repeated the same experiment. We found that the skills that were enabled and their ordering were the exact same in every account. 
From this, we can understand that Alexa opens skills in the order of the highest ratings/reviews if it is not already enabled. The users opinion about which skill to enable is neither asked nor is it properly informed rather than stating the ‘Public name’ of the skill.
To enable a skill that comes later in the ranking, has to be either enabled by visiting the skills store or by multiple enabling and disabling of skills.
If a malicious developer is able to manipulate the ratings/reviews of his skills, the skill would receive a boost in the enablements to end users. This is particularly easy because majority of the skills in the skills store have either no rating or less than 10 ratings. 
Also, the users wouldn’t know which skill they are using unless they checks their Alexa apps on their mobile device.


<  Should we add the actual list of skills we tried out?  >

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%allows duplicate names
%Our testing process is as follows: 

==> userstudy.tex <==
% 
%In this section, we first conduct a comparative analysis of security policies regulated by Amazon Alexa, by comparing them to the policies defined by Google Actions~\cite{PolicyGoogleActions}. Then, we present our brief measurement on the certification system in Google Actions.
\section{User Study}\label{userstudy}

%\cltodo{will move to appendix}

Different from existing user studies that focus on understanding users' security and privacy attitudes towards voice assistants~\cite{ Geeng:2019:WCI, Ammari:2019:MSI, Alexander:2019, Malkin:2019:Privacy, CHI:Eugene:2020}, our study investigates user behaviour about exploring new skills, when encountering something inappropriate, and their trust to VA platforms. We are also interested in how parents manage their kids' usage of VA devices. Answers to these questions will help us understand the risks and serious consequences due to a lack of
trustworthiness of VA platforms.

 


% how users explore new skills, how likely users review a skill (negatively) when encountering something inappropriate, and whether users 

%Misplaced Trust by Users

%seeks to understand users' privacy concerns by conducting a user study. 
%For the user study, we collect, via survey questionnaires, users' security concerns and expectations when interacting with VA devices. 

\subsection{Methodology}

%\ja{hhhhhhh}
%We investigate whether parents' opinions about XXX. 
%{To understand the usage habits of people using Amazon Alexa or Google Assistant at home and their concerns and expectations related to security and privacy, 
	
We conducted an online study using the Amazon Mechanical Turk (MTurk) crowdsourcing platform. We had two groups of users: Amazon Alexa users and Google Assistant users. There were 58 valid users who took part in our survey for Alexa users and 20 valid users who took part in the survey for Google Assistant users. Out of these, 26 of the Alexa users and 6 of the Google Assistant users were parents who have kids under the age of 13.
All the participants in our survey were MTurk masters residing in USA and have
an acceptance rate of at least 98\%. These filters were added to reduce the amount of junk data that we may have collected. All participants were initially presented with a consent form approved by our university's IRB office. Participants who did not consent to the form were denied to proceed with the study. The participants were paid \$0.50 for completing the study.

%To understand how users invoke skills, and XXX, We conduct an online study using the Amazon Mechanical Turk (MTurk) crowdsourcing platform [XX]. In using MTurk, we create survey assignments to XX. In total we have XXX MTurk workers involved in our user study.

%We focus on the following general questions:

\subsection{Response Analysis}

\newcolumntype{L}{>{\centering\arraybackslash}m{3cm}}
\begin{table}[h]
	%\vspace{-6pt}
	%\captionsetup{font=scriptsize}
	\centering
	\resizebox{8.5cm}{!}{
		{
			\begin{tabular}{  >{\arraybackslash}m{5cm} >{\arraybackslash}m{2.3cm} >{\raggedleft\arraybackslash}m{1.1cm}
					>{\raggedleft\arraybackslash}m{1.1cm}}
				\Xhline{5\arrayrulewidth}
				\rowcolor[gray]{0.9} \bf Question & \bf Response & \bf Amazon users & \bf Google users \\
				\hline
				\multirow{2}{*}{\parbox{4cm}{How do you enable new skills? (Alexa specific)}} & Browse the store &  50\% & -\\
				& Enable by voice & \cellcolor{blue!15} 50\%  & -\\
				\hline
				\multirow{3}{*}{\parbox{4.0cm}{Do you usually rate or review skills on the store?}}
				& Yes &  3.45\% & 5\%\\
				& Sometimes & 31.03\% & 30\% \\
				& No & \cellcolor{blue!15} 65.52\%  & \cellcolor{green!15} 65\%\\
				\hline
				
				\multirow{4}{*}{\parbox{4.7cm}{Would you review a skill (negatively) if you encounter something inappropriate?}}
				& Definitely yes & \cellcolor{blue!15} 34.48\% & \cellcolor{green!15} 45\%\\
				& Probably yes & \cellcolor{blue!15} 43.10\% & \cellcolor{green!15} 30\%\\
				& Probably not & 20.69\%  & 20\%\\
				& Definitely no &  1.73\% & 5\%\\
				\hline
				
				\multirow{4}{*}{\parbox{4.5cm}{Do you trust Amazon/Google to detect inappropriate content?}}
				& Definitely yes & \cellcolor{blue!15} 13.79\% & \cellcolor{green!15} 20\%\\
				& Probably yes & \cellcolor{blue!15} 60.35\% & \cellcolor{green!15} 50\%\\
				& Probably not & 25.86\%  & 30\%\\
				& Definitely not & 0\% & 0\%\\
				\hline
				
				\Xhline{5\arrayrulewidth}
			\end{tabular}
		}
	}
	\vspace{-1pt}
	\caption{{Survey responses: general questions}}
	\label{userstudy:general}
	\vspace{-8pt}
\end{table}

%When asked if Google and Amazon should thoroughly test and check the skills before publishing it, 65.52\% of Amazon users and 60\% of Google users responded with definitely yes and another 29.31\% of Amazon users and 40\% of Google users responded with probably yes. 
%The importance of positive social proof and the influence of other people's stories is key in bringing new users to try out the skills. Articles claim that the amount of user reviews have exponentially increased after Amazon rolled out the voice rating feature although a majority of skills are still unrated or have very few ratings on the skills store~\cite{VoiceRatings-Amazon}.

\subsubsection{Usage habits questions}
Table~\ref{userstudy:general} shows the survey responses from Amazon Alexa and Google Assistant
users. We wanted to know which method users chose to explore and enable new skills on their devices. 50\% of the users said that they enable skills by voice while the other 50\% browse the store. This was asked only to the Amazon users because Google does not require the user to enable an action before using it. 65\% of both Alexa and Google users do not rate skills on the store. But when encountering something inappropriate, 78\% of Amazon users and 75\% of Google users tend to rate skills on the skills store. This result suggests that users' negative feedback may help us to identify existing policy-violating skills. When asked if they trusted Amazon and Google to detect and filter out the inappropriate content, 74\% of Amazon users and 70\% of Google users responded with definitely yes or probably yes. These statistics imply that the trust on VA platforms are actually misplaced, and the expectations of the users are not met by Google and Amazon in this regard.

%the percentages of users who responded with definitely yes dropped to 13.79\% and 20\% from Amazon users and Google users respectively. 25.86\% of Amazon users and 30\% of Google users even responded with probably not. 

\iffalse 
\begin{table}[h]
	\vspace{-6pt}
	%\captionsetup{font=scriptsize}
	\centering
	\resizebox{8.9cm}{!}{
		{%\Large
			\begin{tabular}{|c|c|}
			\Xhline{3\arrayrulewidth}
				\rowcolor[gray]{.9} Security/Privacy Concern & Voice Assistant \\
				\hline 
				``I dont know how much they are collecting about me or my kids and what they do with that data'' & Google \\
				\hline 
				``what is being said from the device and i have been hearing that the device is listening in when not in use'' & Google\\
				\hline 
				``That a skill will contain malicious properties if not properly checked'' & Amazon \\
				\hline 
				``That it collects too much personal information'' & Amazon\\
				\hline 
				``To make sure my neices don't stumble onto something inappropriate or adult related''& Amazon \\
				\hline 
				``My activity will be logged and used to develop a file of my interests and schedules'' & Amazon\\
				\hline 
				``Identity theft, inappropriate content for kids'' & Amazon\\
				\Xhline{3\arrayrulewidth}
			\end{tabular}
		}
	}
	\vspace{-1pt}
	\caption{{Survey responses: security and privacy concerns}}
	\label{userstudy:privacyconcerns} 
	\vspace{-6pt}
\end{table}

We also asked an optional question to the users about what their privacy and security concerns are when using these voice assistants. As shown in Table~\ref{userstudy:privacyconcerns}, a majority of users responded with the fear of their voices being recorded and used for purposes that they have not knowingly have provided the consent for. This might be mainly due to awareness about this issue among people after the news reported on Alexa's vulnerabilities. A few users had the fear that the personal information collected would be used inappropriately by the creators and an entire profile of the user will be made from the data. Some parents also feared that their child hears something inappropriate from the device. \\
\fi 

\subsubsection{Parents specific questions}

We asked a few questions specifically to parents who have kids under the age of 13. Table~\ref{userstudy:parents} lists the survey responses. 65\% of Amazon users in our group have provided permission to use kids skills and 23\% were not sure if they did. When asked if they use the Amazon Freetime subscription, only 46\% said yes. While Freetime provides better control to the parents over how their children interacts with Alexa, the number of users making use of the paid subscription is less. Only 31\% of Alexa users extensively test the kids skills at least half the time before enabling it for them.
In the case of Google users, all of them responded that, half the time, they don't check the actions before using them. This shows the trust that users have of Amazon and Google. Also testing every skill extensively before enabling is not feasible from a users' perspective and is something that should be done by the skill certification team before publishing it. 58\% of Alexa users and all of the Google users in our survey had a dedicated VA for their kids. This shows that the parents might not be around with the children to monitor the interactions when the kids use the device.  When asked if the Alexa users check their activities on the Alexa smartphone app, the responses were almost equally divided across the spectrum. While this is a good method to monitor the conversations happening between the VA device and the family members, it can be pretty tiresome to do it on a regular basis. Also, we noticed an inconsistency in the responses that we received from the device and the ones logged in the activities tab on the Alexa smart-phone app. This can be a bug that needs to be rectified (We have reported this bug to the Amazon security team). It does defeat the purpose of the activities tab at this stage. 


\begin{table}[h]
		\vspace{-6pt}
	%\captionsetup{font=scriptsize}
	\centering
	\resizebox{8.5cm}{!}{
		{%\Large
			\begin{tabular}{  >{\arraybackslash}m{5cm} >{\arraybackslash}m{2.3cm} >{\raggedleft\arraybackslash}m{1.1cm}
					>{\raggedleft\arraybackslash}m{1.1cm}}
					\Xhline{3\arrayrulewidth}
				\rowcolor[gray]{0.9} \bf Question & \bf Response & \bf Amazon users & \bf Google users \\
				\hline
				\multirow{2}{*}{\parbox{5cm} {Have you provided the permission to use kids skills on your devices? /\\ Do use Actions for families?}} & Yes & \cellcolor{blue!15} 65.38\% & \cellcolor{green!15} 33.33\%\\
				& No & 11.54\%  & 66.67\%\\
				& Not sure & 23.08\%  & 0\\
				\hline
				\multirow{3}{*}{\parbox{5cm}{Do you use Amazon freetime/ Family Link?}}
				& Yes &  \cellcolor{blue!15} 46.15\% & \cellcolor{green!15} 50\%\\
				& No & 38.46\% & 50\% \\
				& Not sure & 15.39\% &  0\% \\
				\hline
				\multirow{3}{*}{\parbox{5cm}{Do you extensively test kid's skills before enabling it for them?}}
				& Always &  \cellcolor{blue!15} 19.23\% & 0\%\\
				& Most of the time & \cellcolor{blue!15} 11.54\% & 0\% \\
				& About half the time & 7.69\%  & 0\%\\
				& Sometimes &  34.62\% & 50\%\\				
				& Never &  26.92\% & 50\%\\				
				\hline
				
				\multirow{2}{*}{\parbox{5cm}{Do you have a dedicated smart speaker device for your kids?}}
				& Yes &  \cellcolor{blue!15} 57.69\% & 100\%\\
				& No &  42.31\% & 0\%\\
				\hline
				
				\multirow{5}{*}{\parbox{5cm}{How often do you check the activity on your Alexa app? (Alexa specific)}}
				& Always &  16.67\% & -\\
				& Most of the time & 27.77\% & - \\
				& About half the time & 16.67\%  & -\\
				& Sometimes &  \cellcolor{blue!15} 16.67\% & -\\				
				& Never &  \cellcolor{blue!15} 22.22\% & -\\				
			
				\Xhline{3\arrayrulewidth}
			\end{tabular}
		}
	}
	\vspace{-1pt}
	\caption{{Survey responses: parents specific questions}}
	\label{userstudy:parents}
	\vspace{-8pt}
\end{table}


{We had another 16 users who attempted the survey but were not using any voice assistants at home. On asking for the reason for this, 9 of them responded that they feel like it compromises privacy and security.}


